Regular Expressions in a CS Formal Languages Course

Regular expressions in an Automata Theory and Formal Languages course are mostly treated as a theoretical topic. That is, to some degree their mathematical properties and their role to describe languages is discussed. This approach fails to capture the interest of most Computer Science students. It is a missed opportunity to engage Computer Science students that are far more motivated by practical applications of theory. To this end, regular expressions may be discussed as the description of an algorithm to generate words in a language that is easily programmed. This article describes a programming-based methodology to introduce students to regular expressions in an Automata Theory and Formal Languages course. The language of instruction is FSM in which there is a regular expression type. Thus, facilitating the study of regular expressions and of algorithms based on regular expressions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{Elena Machkasova (Ed.): International Workshop on Trends\\
in Functional Programming in Education 2023 (TFPIE 2023)\\
EPTCS 382, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.382.3}{10.4204/EPTCS.382.3}}

